FinRL-Meta: A Universe of Near-Real Market Environments for Data-Driven Deep Reinforcement Learning in Quantitative Finance

Deep reinforcement learning (DRL) has shown huge potentials in building financial market simulators recently. However, due to the highly complex and dynamic nature of real-world markets, raw historical financial data often involve large noise and may not reflect the future of markets, degrading the fidelity of DRL-based market simulators. Moreover, the accuracy of DRL-based market simulators heavily relies on numerous and diverse DRL agents, which increases demand for a universe of market environments and imposes a challenge on simulation speed. In this paper, we present a FinRL-Meta framework that builds a universe of market environments for data-driven financial reinforcement learning. First, FinRL-Meta separates financial data processing from the design pipeline of DRL-based strategy and provides open-source data engineering tools for financial big data. Second, FinRL-Meta provides hundreds of market environments for various trading tasks. Third, FinRL-Meta enables multiprocessing simulation and training by exploiting thousands of GPU cores. Our codes are available online at https://github.com/AI4Finance-Foundation/FinRL-Meta.

==> NeurIPS_2020_version/Section4_Evaluation.tex <==
\section{Evaluation of Trading Performance}

Standard metrics and baseline trading strategies are provided to support trading performance analysis. FinRL library follows a training-validation-testing flow to design a trading strategy. 
%FinRL also considers many trading constraints to perform backtesting tests.

\subsection{Standard Performance Metrics}
FinRL provides five evaluation metrics to help users evaluate the stock trading performance directly, which are final portfolio value, annualized return, annualized standard deviation, maximum drawdown ratio, and Sharpe ratio.

%\textbf{Final portfolio value}: portfolio value at the end of the trading stage.
%
%\textbf{Annualized return}: geometric average amount of money earned by the agent each %year over the time period. 
%
%\textbf{Annualized standard deviation}: annualized standard deviation of the portfolio %return $R_{p}$.
%
%\textbf{Maximum drawdown ratio}: the maximum percentage loss during the trading eriod.
%% FinRL pushes back at any historical point in the selected cycle, then find the nadir %of total assets. 
%
%\textbf{Sharpe ratio:} the average return earned in excess of the risk-free rate per %unit of volatility or total risk:
%\begin{equation}
%\text{Sharpe Ratio} =\frac{\mathbb{E}\left(R_{p}\right)-R_{f}}{\sigma_{p}},
%\end{equation}
%where $\mathbb{E}\left(R_{p}\right)$ is expected return rate, $R_{f}$ is risk-free %rate, and $\sigma_{p}$ is the standard deviation of $R_{p}$. 
 
\subsection{Baseline Trading Strategies}
Baseline trading strategies should be well-chosen and follow industrial standards. The strategies will be universal to measure, standard to compare with, and easy to implement. In FinRL library, traditional trading strategies serve as the baseline for comparing with DRL strategies. Investors usually have two objectives for their decisions: the highest possible profits and the lowest possible risks of uncertainty \cite{sharpe1970portfolio}. FinRL uses five conventional strategies, namely passive buy-and-hold trading strategy \cite{Malkiel2003PassiveIS}, mean-variance strategy \cite{meanvariance2012}, and min-variance strategy \cite{meanvariance2012}, momentum trading strategy \cite{Foltice2015ProfitableMT}, and equal-weighted strategy to address these two mutually limiting objectives and the industrial standards.

%\textbf{Passive Trading Strategy} \cite{Malkiel2003PassiveIS}: is a popular, very easy to implement, and lucrative strategy among investors. With minimal trading activities, investors simply buy and hold index ETFs \cite{Tarassov2016ExchangeTF} to replicate a broad market index or indices. Popular index ETFs are: SPDR S\&P 500 ETF Trust (SPY) and Vanguard 500 Index Fund (VOO) for S\&P 500 Index, SPDR Dow Jones Industrial Average ETF Trust (DIA) for Dow Jones Industrial Average, Invesco QQQ Trust Series 1 (QQQ) for Nasdaq 100 index, etc.

%\textbf{Mean-Variance Strategy} \cite{meanvariance2012}: to achieve an optimal balance between the risks and profits, or the highest Sharpe ratio. The objective of the mean-variance strategy is to minimize risk for a given level of expected return:
%\begin{equation}
%\begin{split}
%&\underset{{w_i}}{\min}~\text{var}(r_p) \\
%&\text{subject~to}~\mathbb{E}(r_p) = \mu^*,~~ \sum w_i = 1,
%
%\end{split}
%\end{equation} where $r_p$ is the portfolio return, $w_i$ is the portfolio weights, and %$\mu^*$ is the expected or target return.

%\textbf{Min-Variance Strategy} \cite{meanvariance2012}: to find the portfolio with the smallest variance. It indicates a well-diversified portfolio that consists of individually risky assets, which are hedged when traded together, resulting in the lowest possible risk for the rate of expected return. The objective function of min-variance model is similar to mean-variance model without setting the target return.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Training-Validation-Testing Flow}

\begin{figure}[t]
\centering
\includegraphics[scale=0.46]{image/data_4.pdf}
\caption{Data splitting.}
\label{data}
\end{figure}


%\begin{figure}[t]
%\centering
%\includegraphics[height=4.5cm]{image/MADDPG515.png}
%\caption{The liquidation process with independent, competitive and cooperative agents using the FinRL library.}
%\label{fig5}
%\vspace{-0.17in}
%\end{figure}

%\begin{figure*}[t]
%\centering
%\includegraphics[height=2.0cm]{image/timeline507.png}
%\caption{Data splitting.}
%\label{fig4}
%\end{figure*}



%\yanglet{To Bruce: need to give reasons about why this flow is necessary for financial tasks?}
With our use cases as instances, the stock market data are divided into three phases in Fig. \ref{data}. Training dataset is the sample of data to fit the DRL model. The model sees and learns from the training dataset. Validation dataset is used for parameter tuning and to avoid overfitting. Testing (trading) dataset is the sample of data to provide an unbiased evaluation of a fine-tuned model. Rolling window is usually associated with the training-validation-testing flow in stock trading because investors and portfolio managers may need to rebalance the portfolio and retrain the model periodically. FinRL provides flexible rolling window selection such as on a daily basis, monthly, quarterly, yearly or by user specified.

%Specifically, with our use cases as instances, the stock market data are divided into three phases in Figure \ref{data}.
%According to the standard workflow in quantitative finance, 

%\textbf{Training phase}: we use data from 01/01/2009 to 09/30/2015 to train the automated trading agents.

%\textbf{Validation phase}: we use data from 10/01/2015 to 12/31/2015 to validate the results and adjust key parameters, such as time slice's size and learning rate.

%\textbf{Testing/Trading phase}: we use data from 01/01/2016 to 05/08/2020 (unseen data) to evaluate the performance of the applications.


%In performance evaluation of RL algorithms, the portfolio value and stock index yield are compared in the form of curve graphs in fig.3), users can see the performance of the algorithm on the DJIA constituents' data. Then specific indicators are shown in Table 1, showing the risks of trading using algorithms.

%From the results of RL, we can conclude that DRL method have better performance on DJIA than traditional investment methods and RL methods. There are also differences among different DRL methods. The evaluation model of FinRL is multi-angled and effective.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Backtesting with Trading Constraints}

In order to better simulate practical trading, we incorporate trading constraints, risk-aversion and automated backtesting tools.

\textbf{Automated Backtesting}.
Backtesting plays a key role in performance evaluation. Automated backtesting tool is preferable because it reduces the human error. In FinRL library, we use the Quantopian pyfolio package \cite{pyfolio} to backtest our trading strategies. This package is easy to use and consists of various individual plots that provide a comprehensive image of the performance of a trading strategy. 

\textbf{Incorporating Trading Constraints}.
Transaction costs incur when executing a trade. There are many types of transaction costs, such as broker commissions and SEC fee. We allow users to treat transaction costs as a parameter in our environments:
\begin{itemize}
    \item Flat fee: a fixed dollar amount per trade regardless of how many shares traded.
    \item Per share percentage: a per share rate for every share traded, for example, 1/1000 or 2/1000 are the most commonly used transaction cost rate for each trade.
\end{itemize}
Moreover, we need to consider market liquidity for stock trading, such as bid-ask spread. Bid-ask spread is the difference between the prices quoted for an immediate selling action and an immediate buying action for stocks. In our environments, we can add the bid-ask spread as a parameter to the stock closing price to simulate real world trading experience. 
%Lastly, in order to address the risk-aversion of various traders, one may add the standard deviation of the portfolio returns into our reward function or simply use the risk-adjusted Sharpe ratio as the reward function.


\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{image/perform_1_3.pdf}
\caption{Performance of single stock trading using PPO in the FinRL library.}
\label{single_stock}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{image/perform_2_3.pdf}
\caption{Performance of multiple stock trading and portfolio allocation using the FinRL library.}
\label{fig3}
\end{figure*}

\begin{table*}[t]
		\centering
		\resizebox{\textwidth}{!}{
		\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}\hline
			2019/01/01-2020/09/23 & SPY  & QQQ&GOOGL & AMZN & AAPL  &  MSFT  &  S\&P 500 \\
			\hline
			Initial value   
			&100,000 &100,000&100,000&100,000&100,000&100,000&100,000\\
			Final value     
			&127,044&163,647&174,825&192,031&173,063&172,797&133,402\\
			Annualized return 
			&14.89\%&32.33\% &37.40\%& 44.94\% &36.88\%&36.49\% &17.81\% \\
			Annualized Std &9.63\%&27.51\%&33.41\%&29.62\%&25.84\%&33.41\%&27.00\%\\
			Sharpe ratio      
			& 1.49 & 1.16& 1.12& 1.40& 1.35 & 1.10 &  0.74   \\
			Max drawdown &20.93\%&28.26\%&27.76\%&21.13\%&22.47\%&28.11\%&33.92\%\\
			\hline
		\end{tabular}}
		\caption{Performance of single stock trading using PPO in the FinRL library. The Sharpe ratio of all the ETFs and stocks outperform the market, namely the S\&P 500 index.}
		\label{single_stock_performance}
	\end{table*}
	
	



\begin{table*}[t]
		\centering
		\resizebox{\textwidth}{!}{
		\begin{tabular}{|l|c|c|c|c|c|}\hline
			2019/01/01-2020/09/23 & TD3 & DDPG&  Min-Var. &  DJIA \\
			\hline
			Initial value   
			&1,000,000 &1,000,000&1,000,000&1,000,000\\
			Final value     
			&\textcolor{orange}{1,403,337};~~\textcolor{cyan}{1,381,120}& \textcolor{orange}{1,396,607};~~\textcolor{cyan}{1,281,120}&1,171,120&1,185,260\\
			Annualized return 
			&\textcolor{orange}{21.40\%}; ~~\textcolor{cyan}{17.61\%}&
			\textcolor{orange}{20.34\%}; ~~\textcolor{cyan}{15.81\%}&8.38\%& 10.61\%\\
			Annualized Std 
			&\textcolor{orange}{14.60\%}; ~~\textcolor{cyan}{17.01\%}&
			\textcolor{orange}{15.89\%};~~\textcolor{cyan}{16.60\%}
			&26.21\%&28.63\%\\
			Sharpe ratio      
			& \textcolor{orange}{1.38}; ~~\textcolor{cyan}{1.03}
			&\textcolor{orange}{1.28}; ~~\textcolor{cyan}{0.98} & 0.44 &0.48  \\
			Max drawdown 
			&\textcolor{orange}{11.52\%}~~\textcolor{cyan}{12.78\%}&
			\textcolor{orange}{13.72\%}; ~~\textcolor{cyan}{13.68\%}&34.34\%&37.01\%\\
			\hline
		\end{tabular}}
		\caption{Performance of \textcolor{orange}{multiple stock trading} and \textcolor{cyan}{portfolio allocation} over the DJIA constituents stocks using the FinRL library. The Sharpe ratios of TD3 and DDPG excceed the DJIA index, and the traditional min-variance portfolio allocation strategy.}
		\label{tab:Performance evaluation}
		\vspace{-0.15in}
	\end{table*}
	
\textbf{Risk-aversion}.
Risk-aversion reflects whether an investor will choose to preserve the capital. It also influences one's trading strategy when facing different market volatility level.

To control the risk in a worst-case scenario, such as financial crisis of 2007–2008, FinRL employs the financial turbulence index $\textit{turbulence}_t$ that measures extreme asset price fluctuation \cite{turbulence}:
\begin{equation}  
\textit{turbulence}_t = \left(\bm{y_t} - \bm{\mu}\right)\bm{\Sigma^{-1}}(\bm{y_t}-\bm{\mu})' \in \mathbb{R},
\label{turb}
\end{equation} 
where $\bm{y_t} \in \mathbb{R}^n$ denotes the stock returns for current period t, $\bm{\mu} \in \mathbb{R}^n$ denotes the average of historical returns, and $\bm{\Sigma} \in \mathbb{R}^{n \times n}$ denotes the covariance of historical returns. It is used as a parameter that controls buying or selling action, for example if the turbulence index reaches a pre-defined threshold, the agent will halt buying action and starts selling the holding shares gradually.



\subsection{Demonstration of Three Use Cases}

We demonstrate with three use cases: single stock trading \cite{Dang2019ReinforcementLI,DRL_automate,li_a2c_2018,zhang2020deep}, multiple stock trading \
\cite{xiong2018practical,yang2020}, and portfolio allocation \cite{Jiang2017ADR,li2019optimistic}. FinRL library provides practical and reproducible solutions for each use case, with online walk-through tutorial using Jupyter notebook (e.g., the configurations of the running environment and commands). We select three use cases and reproduce the results using FinRL to establish a benchmark for the quantitative finance community.

Fig. \ref{single_stock} and Table \ref{single_stock_performance} demonstrate the performance evaluation of single stock trading. We pick large-cap ETFs such as SPDR S\&P 500 ETF Trust (SPY) and Invesco QQQ Trust Series 1 (QQQ), and stocks such as Google (GOOGL), Amazon (AMZN), Apple (AAPL), and Microsoft (MSFT). We use PPO algorithm in FinRL and train a trading agent.  The maximum drawdown in Table \ref{single_stock_performance} is large due to Covid-19 market crash.

Fig. \ref{fig3} and Table \ref{tab:Performance evaluation} show the performance and multiple stock trading and portfolio allocation over the Dow Jones 30 constitutes. We use DDPG and TD3 to trade multiple stocks, and allocate portfolio.




